CancerLLM: A Large Language Model in Cancer Domain

Medical Large Language Models (LLMs) have demonstrated impressive performance on a wide variety of medical NLP tasks; however, there still lacks a LLM specifically designed for phenotyping identification and diagnosis in cancer domain. Moreover, these LLMs typically have several billions of parameters, making them computationally expensive for healthcare systems. Thus, in this study, we propose CancerLLM, a model with 7 billion parameters and a Mistral-style architecture, pre-trained on nearly 2.7M clinical notes and over 515K pathology reports covering 17 cancer types, followed by fine-tuning on two cancer-relevant tasks, including cancer phenotypes extraction and cancer diagnosis generation. Our evaluation demonstrated that the CancerLLM achieves state-of-the-art results with F1 score of 91.78% on phenotyping extraction and 86.81% on disganois generation. It outperformed existing LLMs, with an average F1 score improvement of 9.23%. Additionally, the CancerLLM demonstrated its efficiency on time and GPU usage, and robustness comparing with other LLMs. We demonstrated that CancerLLM can potentially provide an effective and robust solution to advance clinical research and practice in cancer domain

==> experiments_back.tex <==

% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{1\textwidth}{!}{%
% 	\begin{tabular} {l|ccc|ccc|ccc}
% 		\toprule 
% 		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}\\
% 		%\hline
% 		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1  \\
% 	      \midrule
%         % Mamba 2.7 B~\cite{gu2023mamba} &  testing   &     &    &     &    &     &       \\
%         PMC LLaMA 7B~\cite{wu2023pmc} &   81.79  & 36.24   & 50.23  &     &   &     & \\
%          Medalpaca 7B~\cite{han2023medalpaca} & 85.39    &  85.39    &85.39     &     &   &     & \\
%           LLAMA-2 7B~\cite{han2023medalpaca} & 85.86    &  85.86     & 85.86    &     &   &     &  \\
%    Mistral 1*7B~\cite{jiang2023mistral} & 86.53    & 86.53 &  86.53  &     &  &     &   \\
%      Mistral 8*7B~\cite{jiang2023mistral} & \textbf{ 87.10}     &  \textbf{ 87.10}    & \textbf{ 87.10}  &     &   &     &   \\
%       Bio-Mistral 7B~\cite{labrak2024biomistral} &  85.67  &    85.67  &   85.67  &     &  &     & \\
%  LLama3 8B~\cite{} &  85.10 & 85.10&    85.10  &     &   &     &   \\
%                 \hline
%                 MedLLaMA 13B~\cite{wu2023pmc} &   85.75  &  85.67  & 85.71  &     &  &     &  \\
%                 PMCLLaMA 13B~\cite{wu2023pmc} &   84.66  &84.34    &   84.50   &     &  &     & \\
%                 Medalpaca 13B~\cite{han2023medalpaca} &   85.58  &   85.58 & 85.58    &     &  &     &  \\
%                  LLaMA2 13B~\cite{touvron2023llama} &   86.24  &   86.24    & 86.24    &     &  &     &   \\
%                  \hline
%                   LLaMA2 70B~\cite{touvron2023llama} &  86.71     &  86.71        &   86.71   &     &  &     &   \\
%                 MEDITRON-70B~\cite{chen2023meditron} &   model requesting    &        &      &     &   &     & \\
%                 ClinicalCamel-70B~\cite{toma2023clinical} &   model requesting    &        &    &     & &     &  \\
                
%            % Med-Alpaca &     &     &   \\
%            \bottomrule
% 	\end{tabular}
%   }
% \vspace{+2mm}
% \caption{Results of various approaches for pathology report}
% \label{con:Model_pathology}
% \vspace{-1mm}
% \end{table*}








\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1  \\
	      \midrule
        Mamba 2.7 B~\cite{gu2023mamba} &     &     &    &     &    &     &       \\
        PMC LLaMA 7B~\cite{wu2023pmc} &     &     &    &     &   &     & \\
         Medalpaca 7B~\cite{han2023medalpaca} &     &     &    &     &   &     & \\
          LLAMA-2 7B~\cite{han2023medalpaca} &     &     &   &     &   &     &  \\
   Mistral 1*7B~\cite{jiang2023mistral} &     &  &    &     &  &     &   \\
     Mistral 8*7B~\cite{jiang2023mistral} &    &      &    &     &   &     &   \\
      Bio-Mistral 7B~\cite{} &     &     &    &     &  &     & \\
 LLama3 8B~\cite{} &   &   &     &     &   &     &   \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc} &     &   &    &     &  &     &  \\
                PMC LLaMA 13B~\cite{wu2023pmc} &     &    &       &     &  &     & \\
                Medalpaca 13B~\cite{han2023medalpaca} &      &    &      &     &  &     &  \\
                 LLaMA2 13B~\cite{touvron2023llama} &      &        &      &     &  &     &   \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} &      &        &    &     &  &     &   \\
                % MEDITRON-70B~\cite{chen2023meditron} &      &        &      &     &   &     & \\
                   Llama3-OpenBioLLM-70B&   model requesting    &        &      &     &   &     & \\
                ClinicalCamel-70B~\cite{toma2023clinical} &      &        &    &     & &     &  \\
                 Ours~\cite{toma2023clinical} &      &        &    &     & &     &  \\
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of  Cancer Plan}
\label{con:Model_performance_Cancer_plan}
\vspace{-1mm}
\end{table*}



==> experiments_back_5_25.tex <==


\section{Experiments}
\label{experiments}


\subsection{Settings}
We evaluated three state-of-the-art LLMs: LLamA2-13B, MedLLamA-13B, and LLaMA3 8B, along with three retrievers: BM25, TopK-Contriver, and MEdCPT. We considered five biomedical NLP tasks: triple extraction, link prediction, text classification, question answering, and natural language inference, across nine datasets: ADE, ChemProt, GIT, PHarmKG, Hetionet, Ade-corpus-v2, SemedCLass, MedMCQA, and BioNLI. The experiments were conducted using A100 GPUs.



\subsection{Baselines}












\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1  \\
	      \midrule
        % Mamba 2.7 B~\cite{gu2023mamba} &  testing   &     &    &     &    &     &       \\
        PMC LLaMA 7B~\cite{wu2023pmc} &  86.15    &    86.15   &   86.15  & 89.57     & 89.57  & 89.57    & 92.40 & 92.40 & 92.40 \\
         Medalpaca 7B~\cite{han2023medalpaca} & 85.48      &   85.48  &  85.48   &  89.51   &  89.51  &  89.51    & 92.52 & 92.52& 92.52\\
          LLAMA-2 7B~\cite{han2023medalpaca} & 85.86    & 85.86     &85.86      & 89.75    &89.75    &  89.75    & 92.37& 92.37& 92.37  \\
   Mistral 1*7B~\cite{jiang2023mistral} & 86.72    & 86.72    &86.72      &   90.48  &90.48  &   90.48  & 93.26& 93.26 & 93.26    \\
     Mistral 8*7B~\cite{jiang2023mistral} &     \textbf{87.19}   &   \textbf{ 87.19 }   &   \textbf{87.19}   &  \textbf{90.93}    &   \textbf{90.93 } &     \textbf{90.93}  &  \textbf{93.44}    &  \textbf{93.44}   &  \textbf{93.44}  \\
      Bio-Mistral 7B~\cite{labrak2024biomistral} & 85.86   & 85.86      & 85.86      & 89.78    &89.78  &   89.78  &92.67& 92.67& 92.67 \\
 LLama3 8B~\cite{} & 86.15    &    86.15   &   86.15     &   90.27   &  90.27  & 90.27     &92.93 &92.93&92.93  \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc} &   85.86    &   85.86  &  85.86  &     89.43 &89.43  &  89.43   &  92.33  &  92.33 &  92.33  \\
                PMCLLaMA 13B~\cite{wu2023pmc} &  84.72     &  84.72    & 84.72     & 88.26    & 88.26  &    88.26   &91.32 &91.32&91.32 \\
                Medalpaca 13B~\cite{han2023medalpaca} & 85.77      &   85.77  &   85.77  &  89.41    &89.41   &  89.41    & 92.00& 92.00& 92.00  \\
                 LLaMA2 13B~\cite{touvron2023llama} &86.53     &   86.53  & 86.53   &  90.27    & 90.27 & 90.27    & 92.99 & 92.99 & 92.99   \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} &86.72      & 86.72           &   86.72  &   90.44   &  90.44 &   90.44   & 92.81 & 92.81 & 92.81   \\
                % MEDITRON-70B~\cite{chen2023meditron} &   model requesting    &        &      &     &   &     & \\
                Llama3-OpenBioLLM-70B&   running   &        &      &     &   &     & \\
                ClinicalCamel-70B~\cite{toma2023clinical} &   \textbf{88.33}   &  \textbf{88.33}      & \textbf{88.33}    &    92.32  &  92.32&  92.32    &94.25 &94.25 &94.25   \\
                 Ours_test1 & 86.43       & 86.43        &  86.43   &  90.49    &90.49 &  90.49   &92.95&92.95  &92.95     \\
                    Ours &        &        &    &     & &     &  \\
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of various approaches for pathology report}
\label{con:Model_pathology}
\vspace{-1mm}
\end{table*}





\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1  \\
	      \midrule
        % Mamba 2.7 B~\cite{gu2023mamba} &     &     &    &     &    &     &       \\
        PMC LLaMA 7B~\cite{wu2023pmc} &    52.61  &52.61      & 52.61    &  62.11   & 62.11   & 62.11     &71.14 &71.14&71.14 \\
         Medalpaca 7B~\cite{han2023medalpaca} & 55.03    &  55.03    &   55.03  &   63.91  & 63.91 & 63.91&   73.48  &  73.48&  73.48\\
          LLAMA-2 7B~\cite{han2023medalpaca} & 48.48     & 48.48      & 48.48    &  58.83   &  58.83 &   58.83  &69.19 &69.19&69.19 \\
   Mistral 1*7B~\cite{jiang2023mistral} & \textbf{65.45}    &  \textbf{65.45}  &  \textbf{ 65.45}   & \textbf{72.04}     &\textbf{72.04}  &  \textbf{72.04}   &  \textbf{79.13} &  \textbf{79.13} &  \textbf{79.13}  \\
     Mistral 8*7B~\cite{jiang2023mistral} &   51.64 &   51.64   &    51.64&   61.12   & 61.12   &61.12      &  70.53 &  70.53 &  70.53  \\
      Bio-Mistral 7B~\cite{labrak2024biomistral}&62.79      & 62.79     &  62.79  &   70.24   &    70.24   & 70.24& 77.58 & 77.58 & 77.58  \\
 LLama3 8B~\cite{} &55.64    & 55.64  &55.64     & 64.49     &64.49   & 64.49    &  73.90&  73.90&  73.90  \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc} &   56.48   &56.48   &  56.48  &65.54     & 65.54   & 65.54      &   74.29  &   74.29&   74.29\\
                PMC LLaMA 13B~\cite{wu2023pmc} &  59.15    &59.15     &59.15       &  67.20    &     67.20   &  67.20   & 75.66  &75.66 & 75.66\\
                Medalpaca 13B~\cite{han2023medalpaca} &  54.30     &   54.30  &  54.30     & 63.88     & 63.88 & 63.88    & 73.04 & 73.04& 73.04  \\
                 LLaMA2 13B~\cite{touvron2023llama} &  44.12     &    44.12     &  44.12    & 55.24    &  55.24 &  55.24   &  65.37 &  65.37&  65.37  \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} & no running     &        &    &     &  &     &   \\
                % MEDITRON-70B~\cite{chen2023meditron} &      &        &      &     &   &     & \\
                    Llama3-OpenBioLLM-70B&   model requesting    &        &      &     &   &     & \\
                ClinicalCamel-70B~\cite{toma2023clinical} &  no running    &        &    &     & &     &  \\
                 Ours &        &        &    &     & &     &  \\
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of  breast Cancer Diagnosis}
\label{con:Model_performance_Cancer_plan}
\vspace{-1mm}
\end{table*}









\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1  \\
	      \midrule
        PMC LLaMA 7B~\cite{wu2023pmc} &     &     &    &     &   &     & \\
         Medalpaca 7B~\cite{han2023medalpaca} &   41.75   &  41.75    &   41.75  &   50.16  & 50.16  & 50.16    &62.07  &62.07&62.07\\
          LLAMA-2 7B~\cite{han2023medalpaca} &  33.18    &     33.18  &   33.18  & 42.80    &  42.80  &   42.80   & 55.09& 55.09& 55.09  \\
   Mistral 1*7B~\cite{jiang2023mistral} & 45.40    & 45.40 &   45.40 &  54.29    & 54.29   &   54.29    &  65.52  &  65.52&  65.52\\
     Mistral 8*7B~\cite{jiang2023mistral} &    &      &    &     &   &     &   \\
      Bio-Mistral 7B~\cite{} &     &     &    &     &  &     & \\
 LLama3 8B~\cite{} &   &   &     &     &   &     &   \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc} &   39.02   &39.02    & 39.02    &48.98      &  48.98&  48.98   &60.63 &60.63&60.63  \\
                PMC LLaMA 13B~\cite{wu2023pmc} &      &    &       &     &  &     & \\
                Medalpaca 13B~\cite{han2023medalpaca} &      &    &      &     &  &     &  \\
                 LLaMA2 13B~\cite{touvron2023llama} &      &        &      &     &  &     &   \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} &      &        &    &     &  &     &   \\
                % MEDITRON-70B~\cite{chen2023meditron} &      &        &      &     &   &     & \\
                   Llama3-OpenBioLLM-70B&      &        &      &     &   &     & \\
                ClinicalCamel-70B~\cite{toma2023clinical} &      &        &    &     & &     &  \\
                 Ours~\cite{toma2023clinical} &      &        &    &     & &     &  \\
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of  lung  and breast Cancer Diagnosis}
\label{con:Model_performance_Cancer_plan}
\vspace{-1mm}
\end{table*}


% \subsection{Dataset}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|ccc|ccc|ccc}
% 		\toprule 
  
% 		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Breast cancer}& \multicolumn{3}{c}  {lung cancer} & \multicolumn{3}{c}  {other cancer} \\
% 		%\hline
% 		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 \\
   
% 	      \midrule
%                 MedLLaMA 13B~\cite{wu2023pmc} &     &    &     &   &  &  &  &  &  \\
%                  LLaMA2 13B~\cite{touvron2023llama} &     &     &       &     & &    & &   & \\
%                 Mistral-7B~\cite{jiang2023mistral} &     &     &       &     & &    & &   & \\
%                  Mamba 2.7 B~\cite{gu2023mamba} &     &     &       &     & &    & &   & \\
%            Med-Alpaca &     &     &       &     & &    & &   & \\
           
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for cancer QA, few-shot result}
% \label{con:Model_performance_Chem_DDI_GIT}
% \vspace{-1mm}
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|ccc|ccc|ccc}
% 		\toprule 
  
% 		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Breast cancer}& \multicolumn{3}{c}  {lung cancer} & \multicolumn{3}{c}  {other cancer} \\
% 		%\hline
% 		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 \\
   
% 	      \midrule
%                 MedLLaMA 13B~\cite{wu2023pmc} &     &    &     &   &  &  &  &  &  \\
%                  LLaMA2 13B~\cite{touvron2023llama} &     &     &       &     & &    & &   & \\
%                 Mistral-7B~\cite{jiang2023mistral} &     &     &       &     & &    & &   & \\
%                  Mamba 2.7 B~\cite{gu2023mamba} &     &     &       &     & &    & &   & \\
%            Med-Alpaca &     &     &       &     & &    & &   & \\
           
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for cancer QA, zero-shot result}
% \label{con:Model_performance_Chem_DDI_GIT}
% \vspace{-1mm}
% \end{table*}







\subsection{Results and Discussion}
\label{con:discussuion_triple}




\subsection{Analysis}


% \begin{figure}[t]
%         \centering
%         \includegraphics[width=0.98\columnwidth]{chuck_number.pdf}
% 	\caption{  \textsc{PeTailor} performance with different  chunk length ($m$) in the triple extraction task. P is Precision, R is Recall and F is F1-score.
%  }
% 	\label{con:chunk_number_triple}
% \end{figure}


\subsubsection{Ablation Experiments}



==> result_back.tex <==


\section{Experiments}
\label{experiments}


\subsection{Settings}
We evaluated three state-of-the-art LLMs: LLamA2-13B, MedLLamA-13B, and LLaMA3 8B, along with three retrievers: BM25, TopK-Contriver, and MEdCPT. We considered five biomedical NLP tasks: triple extraction, link prediction, text classification, question answering, and natural language inference, across nine datasets: ADE, ChemProt, GIT, PHarmKG, Hetionet, Ade-corpus-v2, SemedCLass, MedMCQA, and BioNLI. The experiments were conducted using A100 GPUs.


\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {c|c|c|ccc|ccc|ccc|ccc}
		\toprule 
  
	\multicolumn{1}{c}  {}&\textbf{}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {triple}& \multicolumn{3}{c}  {head entity }& \multicolumn{3}{c}  {relation} &\multicolumn{3}{c}{tail entity} \\
		%\hline
   Dataset&LLM &Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 \\ 
   \hline
   \multirow{12}{*}{ADE}
    & \multirow{4}*{LLaMA2-13B}&BM25~\cite{luo2023dr} & 30.99 &   30.88  & 30.93  &  73.96  &  73.71  & 73.84 & 94.85 & 94.54 & 94.70 & 49.10 & 48.94 & 49.02 \\
    & &   Contriever~\cite{izacard2021unsupervised}& \cellcolor{green!40} \textbf{\underline{36.07}} &  \cellcolor{green!40}\textbf{\underline{36.06} }&\cellcolor{green!40}\textbf{\underline{36.06}} & 79.76 & 79.72 & 79.74  & 93.80 & 93.76 & 93.78 & 48.99 & 48.97 & 48.98 \\
    &  &MedCPT~\cite{su2023one} &30.81 & 30.80 & 30.81 & 76.75 & 76.71 & 76.73 & 94.41 & 94.37 & 94.39 & 43.87 & 43.85 & 43.86\\ 
            % &random&  train& 45.12 & 45.12 & 45.12 & 83.43 & 83.43 & 83.43 & 96.10 & 96.10 & 96.10 & 54.27 & 54.27 & 54.27 \\
    &  &No Retriever& 34.94 & 34.79 & 34.86 & 83.64 & \underline{83.29} & \underline{83.46} & 95.29 & 94.88 & 95.08 & 42.10 & 41.92 & 42.01 \\
              % \cmidrule(lr){2-15}
   \cmidrule(rr){2-15}

            
   &\multirow{4}*{MedLLaMA-13B}&BM25~\cite{luo2023dr} & 33.77 & 33.76 & 33.77 & 77.06 & 77.02 & 77.04 & 94.82 & 94.77 & 94.80 & \underline{51.20 }& \underline{51.18} & \underline{51.19}  \\
    & &Contriever~\cite{izacard2021unsupervised}& 35.66 & 33.57 & 34.58 & 79.15 & 74.51 & 76.76 & 94.36 & 88.83 & 91.51 & 49.18 & 46.29 & 47.69\\
    &  & MedCPT~\cite{su2023one} & 33.30 & 29.72 & 31.41 & 79.01 & 70.52 & 74.52 & 95.48 & 85.21 & 90.05 & 45.77 & 40.85 & 43.17\\ 
               % &random&train & 39.53 & 39.44 & 39.48 & 82.26 & 82.07 & 82.16 & 95.25 & 95.02 & 95.14 & 48.80 & 48.69 & 48.74 \\
    &  &No Retriever& 12.26 & 12.16 & 12.21 & 81.87 & 81.22 & 81.55 & 95.69 & \underline{94.93} & \underline{95.31} & 15.66 & 15.54 & 15.60 \\
    \cmidrule(rr){2-15}
    & \multirow{4}*{LLaMA3-8B}&BM25~\cite{luo2023dr} & 27.88 & 27.70 & 27.79 & 72.87 & 72.39 & 72.63 & 94.61 & 93.99 & 94.30 & 45.79 & 45.49 & 45.64\\
    & &Contriever~\cite{izacard2021unsupervised}&34.44 & 31.13 & 32.70 & 78.91 & 71.31 & 74.92 & 93.14 & 84.18 & 88.43 & 48.57 & 43.90 & 46.12\\
    &  &MedCPT~\cite{su2023one} & 31.70 & 27.04 & 29.19 & 77.99 & 66.53 & 71.80 & 94.00 & 80.19 & 86.55 & 45.35 & 38.69 & 41.75\\ 
                % &random&  train &  38.62 & 38.31 & 38.46 & 81.64 & 80.99 & 81.31 & 95.41 & 94.65 & 95.03 & 48.56 & 48.17 & 48.36 \\
    &   &No Retriever& 9.85 & 5.49 & 7.05 & \underline{83.84} & 46.76 & 60.04 &\underline{ 96.30} & 53.71 & 68.96 & 13.05 & 7.28 & 9.34  \\   
    \cmidrule(rr){1-15}
    \multirow{12}{*}{ChemProt}
     &  \multirow{4}*{LLaMA2-13B}&BM25~\cite{luo2023dr} & 49.44 & 48.78 & 49.11 & 65.77 & 64.89 & 65.33 & 75.56 & 74.55 & 75.05 & 65.51 & 64.63 & 65.07   \\
    &&TopK-Contriever~\cite{izacard2021unsupervised}&  85.75 & 85.05 & 85.40 & 98.42 & \underline{97.61} & \underline{98.01} & 91.58 & \underline{90.84} & \underline{91.21} & 94.02 & 93.25 & 93.63   \\
    & &MedCPT~\cite{su2023one} & 86.25 & 85.40 & 85.82 &\underline{ 98.44} & 97.47 & 97.95 & 91.19 & 90.29 & 90.73 & \underline{95.53} & 94.59 & 95.06  \\ 
                % &random& train &    89.97 & 89.21 & 89.59 & 98.83 & 97.99 & 98.41 & 92.67 & 91.88 & 92.27 & 97.36 & 96.54 & 96.95\\
    & &No Retriever&   78.58 & 76.41 & 77.48 & 98.12 & 95.40 & 96.74 & 90.70 & 88.19 & 89.43 & 88.21 & 85.78 & 86.98 \\
    \cmidrule(rr){2-15}
     & \multirow{4}*{MedLLaMA-13B}&BM25~\cite{luo2023dr} & 54.78 & 49.53 & 52.02 & 73.30 & 66.29 & 69.62 & 78.10 & 70.62 & 74.17 & 74.40 & 67.28 & 70.66 \\
    & &TopK-Contriever~\cite{izacard2021unsupervised}& 86.15 & 85.22 & 85.69 & 97.97 & 96.92 & 97.44 & 91.38 & 90.40 & 90.89 & 95.18 & 94.15 & 94.66 \\
    & & MedCPT~\cite{su2023one} & 81.33 & 80.08 & 80.70 & 98.14 & 96.63 & 97.38 & 89.60 & 88.22 & 88.91 & 91.96 & 90.55 & 91.25 \\ 
               % &random& train &  88.18 & 87.46 & 87.82 & 98.56 & 97.76 & 98.16 & 91.35 & 90.61 & 90.98 & 97.21 & 96.42 & 96.82  \\
                % &no example zaifu&  --& 77.90 & 76.88 & 77.38 & 98.11 & 96.83 & 97.47 & 89.60 & 88.42 & 89.01 & 87.44 & 86.30 & 86.87 \\
    & &No Retriever&  52.10  &49.04   & 50.52  &  97.65 &  91.91 & 94.69  & 90.82  & 85.48  &88.07  &  57.91 & 54.50  &   56.15\\
                
    \cmidrule(rr){2-15}
    & \multirow{4}*{LLaMA3-8B}&BM25~\cite{luo2023dr} & 70.23 & 69.98 & 70.10 & 83.86 & 83.57 & 83.71 & 84.30 & 84.00 & 84.15 & 91.54 & 91.22 & 91.38  \\
    &  &  Contriever~\cite{izacard2021unsupervised}&\cellcolor{green!40} \textbf{\underline{87.13 }}&\cellcolor{green!40} \textbf{\underline{86.68}} & \cellcolor{green!40} \textbf{\underline{86.91} }& 97.92 & 97.41 & 97.67 & 91.26 & 90.78 & 91.02 & 95.56 & \underline{95.06} & \underline{95.30} \\
    & &MedCPT~\cite{su2023one} & 86.62 & 83.07 & 84.81 & 98.06 & 94.04 & 96.01 &\underline{ 92.54} & 88.74 & 90.60 & 94.06 & 90.20 & 92.09 \\
                % &random& train &   88.00 & 86.56 & 87.27 & 98.11 & 96.51 & 97.30 & 92.05 & 90.55 & 91.29 & 96.24 & 94.68 & 95.45   \\
    & &No Retriever& 23.21 & 19.72 & 21.32 & 98.63 & 83.80 & 90.61 & 91.75 & 77.95 & 84.29 & 26.09 & 22.16 & 23.97  \\
    \hline
    \multirow{12}{*}{GIT} & \multirow{4}*{LLaMA2-13B}&BM25~\cite{luo2023dr} & 60.81 & 54.73 & 57.61 & 76.94 & 69.25 & 72.89 & 76.70 & 69.03 & 72.67 & 77.78 & 70.00 & 73.68 \\
    & &Contriever~\cite{izacard2021unsupervised}& 74.78 & 72.37 & 73.55 & 89.44 & 86.56 & 87.98 & \underline{83.22} & 80.54 & 81.86 & 87.11 & 84.30 & 85.68\\
    &  &MedCPT~\cite{su2023one} & 75.64 & 73.44 & 74.52 & \underline{92.03 }& \underline{89.35} & \underline{90.67} & 83.06 & 80.65 & 81.83 & 89.04 & 86.45 & 87.73 \\ 
             % &random&train&72.14  &  70.75   & 71.44  &  88.37  & 86.66    & 87.51    & 81.57   & 80.00   &80.78    &  86.62  & 84.94&85.77  \\
    &   &No Retriever&  61.76 & 56.45 & 58.99 & 84.12 & 76.88 & 80.34 & 73.53 & 67.20 & 70.22 & 82.94 & 75.81 & 79.21 \\
    \cmidrule(rr){2-15}
    &  \multirow{4}*{MedLLaMA-13B}&BM25~\cite{luo2023dr} &58.59 & 57.20 & 57.89 & 79.30 & 77.42 & 78.35 & 72.91 & 71.18 & 72.03 & 78.63 & 76.77 & 77.69 \\
    & &Contriever~\cite{izacard2021unsupervised}& 65.95 & 65.81 & 65.88 & 85.34 & 85.16 & 85.25 & 75.86 & 75.70 & 75.78 & 83.84 & 83.66 & 83.75 \\
   &  &  MedCPT~\cite{su2023one} & \cellcolor{green!40} \textbf{\underline{75.65}} &\cellcolor{green!40}  \textbf{\underline{74.84}} & \cellcolor{green!40} \textbf{\underline{75.24}} & 90.22 & 89.25 & 89.73 & 82.39 & 81.51 & 81.95 & \underline{90.00 }& \underline{89.03 }& \underline{89.51}  \\ 
              % &random& train&58.70  &36.98     & 45.38  &  90.44  &56.99     & 69.92    & 83.27   & 52.47   &   64.37 & 69.28   & 43.65&53.56  \\
    &   &No Retriever&  42.60 & 41.51 & 42.05 & 89.18 & 86.88 & 88.02 & 75.28 & 73.33 & 74.29 & 52.76 & 51.40 & 52.07 \\
    \cmidrule(rr){2-15}
    &  \multirow{4}*{LLaMA3-8B}&BM25~\cite{luo2023dr} &62.72 & 62.58 & 62.65 & 79.31 & 79.14 & 79.22 & 79.74 & 79.57 & 79.66 & 77.80 & 77.63 & 77.72  \\
    &   &Contriever~\cite{izacard2021unsupervised}&74.76 & 67.53 & 70.96 & 89.76 & 81.08 & 85.20 & 82.14 & 74.19 & 77.97 & 88.33 & 79.78 & 83.84\\
    & &MedCPT~\cite{su2023one} & 66.20 & 50.97 & 57.59 & 87.15 & 67.10 & 75.82 & 82.96 & 63.87 & 72.17 & 78.77 & 60.65 & 68.53 \\ 
              % &random&train  &  75.48 & 75.48 & 75.48 & 87.63 & 87.63 & 87.63 & 82.80 & 82.80 & 82.80 & 87.63 & 87.63 & 87.63  \\
     & &No Retriever&  75.81 & 72.80 & 74.27 & 87.79 & 84.30 & 86.01 & 85.55 & \underline{82.15} & \underline{83.82} & 86.67 & 83.23 & 84.91 \\
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for triple extraction on ADE, ChemProt, and GIT. Underline indicates the best performance on each dataset, while bold font highlights the best F1 performance on each dataset. }
\label{con:triple_extraction_performance}
 
\end{table*}





\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
\Huge
	\begin{tabular} {l|c|ccc|ccc|ccc|ccc|ccc|c}
		\toprule 
    &\multicolumn{1}{c}  {}&\multicolumn{6}{c}  {Link Prediction}&\multicolumn{6}{c}  {Text Classification}&\multicolumn{3}{c}  {Question Answering}&\multicolumn{1}{c}  {Natural Language Inference}\\ 
      \cmidrule(rr){3-8}\cmidrule(rr){9-14}\cmidrule(rr){15-17} \cmidrule(rr){18-18}
		&\multicolumn{1}{c}  {}&\multicolumn{3}{c}{PHarmKG}& \multicolumn{3}{c}{Hetionet}& \multicolumn{3}{c}{Ade-corpus-v2}& \multicolumn{3}{c}{SemClass}  & \multicolumn{3}{c}{MedMCQA} &\multicolumn{1}{c}{BioNLI} \\
		%\hline
		  LLM&Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 & Precision &  Recall & F1 &  Precision &  Recall & F1 & Precision &  Recall & F1&  Macro-avg F1 \\ 	
   
	      \midrule
              \multirow{4}*{LLaMA2-13B}&BM25~\cite{luo2023dr}  & 97.60   & 97.60      &97.60     & 82.37   & 82.37    &82.37  & 95.40  &95.40      & 95.40   &  75.50  &   75.50   &  75.50   &  40.38  &  40.49   & 40.42 & 45.10  \\
            &Contriever~\cite{izacard2021unsupervised} &  \cellcolor{green!40} \textbf{\underline{ 98.00}}   &  \cellcolor{green!40} \textbf{\underline{ 98.00} }   &  \cellcolor{green!40}\textbf{\underline{98.00 } } &   77.00& 77.00    & 77.00& 96.60   & 96.60     &  96.60  &  \cellcolor{green!40} \textbf{\underline{79.33}}  &     \cellcolor{green!40} \textbf{\underline{79.33 }}&    \cellcolor{green!40} \textbf{ \underline{79.33}}   &  35.53  &  35.52   &  35.52  &  35.12  \\
            & MedCPT~\cite{li2023petailor}&   97.40  &  97.40    &  97.40&  81.60  &  81.60   &  81.60 & \cellcolor{green!40}\textbf{ \underline{96.80 }  } &   \cellcolor{green!40}\textbf{\underline{96.80} }  & \cellcolor{green!40}\textbf{ \underline{96.80} }  & 78.50    &  78.50    &     78.50&  36.78  &  36.93   &  36.80  &  \cellcolor{green!40}\textbf{\underline{ 69.21 }}\\
             % &random &  train &testing  &     &   & 79.88   &  79.88   & 79.88   \\
              &No Retriever &  97.60  &   97.60  & 97.60  &  80.80  &  80.80   &  80.80 & 96.40  & 96.40    &  96.40 &   77.66  & 77.66   & 77.66& ---   &     & &      62.62 \\
            \hline
               \multirow{4}*{MedLLaMA-13B}&BM25~\cite{luo2023dr} & 95.00   &   95.00    &    95.00 &  \cellcolor{green!40} \textbf{ \underline{90.40 }}& \cellcolor{green!40}\textbf{\underline{ 90.40 } }  &   \cellcolor{green!40}\textbf{\underline{ 90.40} } & 95.60   & 95.60    &  95.60 &  72.67  &   72.67  &   72.67 &  37.81  & 37.96    &  37.86 &    48.81\\
            &Contriever~\cite{izacard2021unsupervised}&  97.00  &    97.00  &   97.00  &   77.20 &  77.20   &   77.20  &  95.60  &  95.60   &  95.60 &  77.66 & 77.66   & 77.66&  29.82  &   29.75  &  29.77&      53.07  \\
            & MedCPT~\cite{li2023petailor}&     97.40    &   97.40     &  97.40      &   84.40 &   84.40  &   84.40 & 95.40 & 95.40    & 95.40  &76.16    &  76.16    &   76.16&  33.86  &  34.04   &  33.88 &    53.68 \\
             % &random &  train &  running &     &   &    &     &    \\
               &No Retriever &  97.20  &  97.20    &97.20   &  78.54  &  78.54   &  78.54 & 95.40  &  95.40   & 95.40  &   64.00 &    64.00 &  64.00  &    &     & &    61.07 \\
             \hline
        \multirow{4}*{LLaMA3-8B}&BM25~\cite{luo2023dr}   & 96.80  & 96.80    &  96.80 &  81.80  &   81.80  &   81.80&94.80   & 94.80    & 94.80   & 75.50  &   75.50    &  75.50  &  37.73  &  38.90   & 37.79 & 19.17 \\
            &Contriever~\cite{izacard2021unsupervised}&  96.60   &   96.60    &  96.60  &  73.40  &  73.40   &   73.40& 94.60  &  94.60    & 94.60   &   75.83 &  75.83 &75.83&  28.11  &  28.12   &  28.11 & 63.85 \\
            & MedCPT~\cite{li2023petailor} &  97.00  &  97.00   & 97.00   & 83.00   &   83.00  &  83.00 & 95.40 & 95.40    & 95.40  & 74.67 &  74.67   & 74.67&  31.57  &  31.82   &  31.56 &  56.89   \\
             % &random &  train & testing   &     &   & 80.29   &  80.29    & 80.29    \\
               &No Retriever &  97.20 & 97.20    &  97.20 &   81.80 &  81.80   &   81.80&93.80   & 93.80      & 93.80    &   73.16 &   73.16   &  73.16  &    &     & & 6.71 \\
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for link prediction, text classification, question answering, and natural language inference.  Underline with bold font indicates the best performance on each dataset.}
\label{con:Model main performance}
 
\end{table*}





\begin{table*}[ht]
      \Huge
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {c|ccc|ccc|ccc|ccc|ccc}
		\toprule 
        
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ADE} &\multicolumn{3}{c}  {ChemProt} &\multicolumn{3}{c}  {GIT} &\multicolumn{3}{c}  {PHarmKG}&\multicolumn{3}{c}  {Hetionet}\\
		%\hline
		 Corpus & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 \\ 
   \hline
       Unlabeled corpus& 9.76 & 9.53 & 9.65 &   75.56 & 69.14 & 72.21    & 2.29 & 0.65 & 1.01 & 97.20    &97.20 &   97.20 &-&-&-\\
            Labeled corpus &\textbf{36.07} & \textbf{36.06} & \textbf{36.06}&87.13 & 86.68 & \textbf{86.91}  & 75.65 & 74.84 & \textbf{75.24} & 98.00  & 98.00 & 98.00&90.40   &90.40&90.40 \\\
               None& 34.94 & 34.79 & 34.86  &42.60 & 41.51 & 42.05&42.60 & 41.51 & 42.05 &97.60  & 97.60 & 97.60 &78.54 &78.54 &78.54 \\

                   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{RAG Performance for ADE, ChemProt, GIT, PHarmKG  and Hetionet on \textbf{Testbed1 labeled database requirement}. For each dataset, the RAG is the model have the best performance. Such as, on ADE, RAG is LLaMA2-13B with Contriever. Labeled corpus is the training set for each dataset. The unlabeled corpus refers to a training set devoid of labels for each dataset. } 
\label{con:Model main performance_testbed1_0}
 
\end{table*}



\begin{table*}[ht]
      \Huge
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|c}
		\toprule 
        
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ade-corpus-v2}&\multicolumn{3}{c}  {SemClass}&\multicolumn{3}{c}  {MedQA}&\multicolumn{1}{c}  {BioNLI}\\
		%\hline
		Corpus &  Precision &  Recall & F1& Precision &  Recall & F1 & Precision &  Recall & F1 &F1\\ 
   \hline
       Unlabeled corpus&94.80 &94.80&94.80&6.83 &6.83 &6.83  &-&-&-&10.91\\
             Labeled corpus&96.80 & 96.80& 96.80  &79.33 &79.33 &79.33 &40.38 &40.49 &40.42&69.21\\\
               None&96.40&96.40&96.40&77.66& 77.66&77.66&-&-&-&62.62 \\

                   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{RAG Performance for ade-corupus-v2, semCLass, MEdQA, and BIoNL on \textbf{Testbed1 labeled database requirement}. }
\label{con:Model main performance_testbed1_1}
 
\end{table*}






\begin{table*}[ht]
      \Huge
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {c|ccc|ccc|ccc|ccc|ccc}
		\toprule 
        
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ADE} &\multicolumn{3}{c}  {ChemProt} &\multicolumn{3}{c}  {GIT} &\multicolumn{3}{c}  {PHarmKG}&\multicolumn{3}{c}  {Hetionet}\\
		%\hline
		 Corpus & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 \\ 
   \hline
        Counterfactual corpus (20\%) &  41.41 & 41.31 & 41.36 & 74.22& 66.90&70.37 &74.50&71.61& 73.03 & 97.40  & 97.40& 97.40& --&--& --\\
        Counterfactual corpus (80\%) &  41.94 & 36.90 & 39.26  &82.96&33.57&47.79&74.84 &74.84 &74.84&97.80&97.80&97.80& --&--& --  \\
        Counterfactual corpus (100\%) &  25.60 & 25.59 & 25.59 & 84.12 &83.07&83.59&75.22& 74.41& 74.81&97.60 &97.60&97.60& --&--& --\\
            Labeled corpus &\textbf{36.07} & \textbf{36.06} & \textbf{36.06}&87.13 & 86.68 & \textbf{86.91}  & 75.65 & 74.84 & \textbf{75.24} & 98.00  & 98.00 & 98.00&90.40   &90.40&90.40 \\\
               None& 34.94 & 34.79 & 34.86  &42.60 & 41.51 & 42.05&42.60 & 41.51 & 42.05 &97.60  & 97.60 & 97.60 &78.54 &78.54 &78.54 \\
                   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{RAG Performance for ADE, ChemProt, GIT, PHarmKG  and Hetionet on \textbf{Testbed2 counterfactual robustness}. For each dataset, the RAG is the model that has the best performance. Such as, on ADE, RAG is LLaMA2-13B with Contriever. Labeled corpus is the training set for each dataset. 
The 20/80/100\% denotes a training set where 20/80/100\% of instances are mislabeled for each dataset. } 
\label{con:Model main performance_testbed1_0}
 
\end{table*}



\begin{table*}[ht]
      \Huge
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|c}
		\toprule 
        
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ade-corpus-v2}&\multicolumn{3}{c}  {SemClass}&\multicolumn{3}{c}  {MedQA}&\multicolumn{1}{c}  {BioNLI}\\
		%\hline
		Corpus &  Precision &  Recall & F1& Precision &  Recall & F1 & Precision &  Recall & F1 &F1\\ 
   \hline
        Counterfactual corpus (20\%)&95.80   &95.80   &95.80 & 73.33 & 73.33  & 73.33 & --&-- &  --& 47.76 \\
    Counterfactual corpus (80\%)&95.00   &95.00   &95.00 &75.66 &75.66 &75.66 & --& --& -- & 64.63 \\
        Counterfactual corpus (100\%)&96.80   &96.80   &96.80 &77.66 &77.66 &77.66 &-- & --& -- & 46.46\\
        
             Labeled corpus&96.80 & 96.80& 96.80  &79.33 &79.33 &79.33 &40.38 &40.49 &40.42&69.21\\\
               None&96.40&96.40&96.40&77.66& 77.66&77.66&-&-&-&62.62 \\

                   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{RAG Performance for ade-corupus-v2, semCLass, MEdQA, and BIoNL on \textbf{Testbed2 counterfactual robustness}. }
\label{con:Model main performance_testbed1_1}
 
\end{table*}



% \begin{table*}[ht]
%       \Huge
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.5\textwidth}{!}{%
% 	\begin{tabular} {l|c|ccc}
% 		\toprule 
        
% 		\textbf{Dataset}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {triple} \\
% 		%\hline
% 		 &Corpus & Precision &  Recall & F1 \\ 
%    \hline
%         \multirow{3}*{ADE}&Unlabeled corpus& 9.76 & 9.53 & 9.65  \\
%                &LLaMA2-13B Contriever&\textbf{36.07} & \textbf{36.06} & \textbf{36.06}  \\
%                &LLaMA2-13B No Retriever& 34.94 & 34.79 & 34.86  \\
%             \hline
%              \multirow{3}*{ChemProt}&Unlabeled corpus&   75.56 & 69.14 & 72.21   \\
             
%                &LLaMA3-8B Contriever&87.13 & 86.68 & \textbf{86.91} \\
%                 &LLaMA3-8B No Retriever&23.21 & 19.72 & 21.32\\
%             \hline
%              \multirow{3}*{GIT}&Unlabeled corpus&    2.29 & 0.65 & 1.01  \\
%                 & MedLLaMA-13B MedCPT & 75.65 & 74.84 & \textbf{75.24}   \\ 
%                    & MedLLaMA-13B No Retriever &42.60 & 41.51 & 42.05  \\ 
%   \hline
%               \multirow{3}*{PHarmKG}&Unlabeled corpus& 97.20    &97.20 &   97.20   \\
%                 & LLaMA2-13B Contriever & 98.00  & 98.00 & 98.00   \\ 
%                    & LLaMA2-13B No Retriever &97.60  & 97.60 & 97.60 \\ 
                   
%            \bottomrule
% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for four testbed}
% \label{con:Model main performance}
 
% \end{table*}




\begin{table*}[ht]
      \Huge
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {c|ccc|ccc|ccc|ccc|ccc}
		\toprule 
        
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ADE} &\multicolumn{3}{c}  {ChemProt} &\multicolumn{3}{c}  {GIT} &\multicolumn{3}{c}  {PHarmKG}&\multicolumn{3}{c}  {Hetionet}\\
		%\hline
		 Corpus & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 \\ 
   \hline
       Diversity labeled corpus& 11.21& 9.15&10.08 &78.56& 76.41&77.47 &74.88 & 65.38& 69.80 &97.20&97.20&97.20&-&-&-\\
            Labeled corpus &\textbf{36.07} & \textbf{36.06} & \textbf{36.06}&87.13 & 86.68 & \textbf{86.91}  & 75.65 & 74.84 & \textbf{75.24} & 98.00  & 98.00 & 98.00&90.40   &90.40&90.40 \\\
               None& 34.94 & 34.79 & 34.86  &42.60 & 41.51 & 42.05&42.60 & 41.51 & 42.05 &97.60  & 97.60 & 97.60 &78.54 &78.54 &78.54 \\

                   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{RAG Performance for ADE, ChemProt, GIT, PHarmKG  and Hetionet on \textbf{Testbed3 diversity robusteness}. For each dataset, the RAG is the model have the best performance. Such as, on ADE, RAG is LLaMA2-13B with Contriever. Labeled corpus is the training set for each dataset. The unlabeled corpus refers to a training set devoid of labels for each dataset. } 
\label{con:Model main performance_testbed1_0}
 
\end{table*}



\begin{table*}[ht]
      \Huge
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|c}
		\toprule 
        
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ade-corpus-v2}&\multicolumn{3}{c}  {SemClass}&\multicolumn{3}{c}  {MedQA}&\multicolumn{1}{c}  {BioNLI}\\
		%\hline
		Corpus &  Precision &  Recall & F1& Precision &  Recall & F1 & Precision &  Recall & F1 &F1\\ 
   \hline
       Diversity labeled corpus&96.20 & 96.20&96.20 & 75.33 & 75.33 &75.33& --&---&---&80.32 \\
             Labeled corpus&96.80 & 96.80& 96.80  &79.33 &79.33 &79.33 &40.38 &40.49 &40.42&69.21\\\
               None&96.40&96.40&96.40&77.66& 77.66&77.66&-&-&-&62.62 \\

                   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{RAG Performance for ade-corupus-v2, semCLass, MEdQA, and BIoNL on \textbf{Testbed 3 diversity robusteness}. }
\label{con:Model main performance_testbed1_1}
 
\end{table*}





\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.7\textwidth}{!}{%
	\begin{tabular} {l|l|c|c}
		\toprule 
  
		  Task&Dataset & true negative awareness rate &fake negative awareness rate\\ 
    \hline
            \multirow{3}*{triple extraction}&ADE&   1.07 & 9.15   \\
	                  & ChemProt&  19.24 & 77.49\\
                       &GIT&  27.73 & 69.75 \\
             \hline
             \multirow{2}*{link prediction}&PHarmKG&  0.00 & 63.11  \\
	           & Hetionet&   & \\
            \hline
            \multirow{2}*{text classification}&Ade-corpus-v2& 68.75    &  70.45  \\
	     & SemClass&1.49   &  99.35  \\
         \hline
             \multirow{1}*{question answering} & MedMCQA&     &    \\
          % \cmidrule(rr){2-4}
             \hline
           \multirow{1}*{natural language inference} &  BioNLI&   0 &0.38   \\
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for negative awareness rate}
\label{con:Model main performance}
 
\end{table*}


% \begin{table*}[ht]
%       \Huge
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.5\textwidth}{!}{%
% 	\begin{tabular} {l|c|ccc}
% 		\toprule 
        
% 		\textbf{Dataset}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {triple} \\
% 		%\hline
% 		 &Corpus & Precision &  Recall & F1 \\ 
%    \hline
%         \multirow{4}*{ADE}&Unlabeled corpus& 9.76 & 9.53 & 9.65  \\
         
%           &Counterfactual corpus (20\%) &  41.41 & 41.31 & 41.36    \\
%               &Counterfactual corpus (80\%) &  41.94 & 36.90 & 39.26    \\
%               &Counterfactual corpus (100\%) &  25.60 & 25.59 & 25.59  \\
%              &Diversity labeled corpus&  11.21 & 9.15 & 10.08   \\
%               % &NNegative Awareness(all noise test&  25.60 & 25.59 & 25.59 & 65.85 & 65.82 & 65.84 & 65.15 & 65.12 & 65.13 & 37.48 & 37.46 & 37.47  \\
%                &LLaMA2-13B Contriever&\textbf{36.07} & \textbf{36.06} & \textbf{36.06}  \\
%                &No Retriever& 34.94 & 34.79 & 34.86  \\
%             \hline
%              \multirow{4}*{ChemProt}&Labeled Database Requirement&   75.56 & 69.14 & 72.21   \\
%               &Counterfactual Robustness rate 0.2 &  74.22 & 66.90 & 70.37\\
%               &Counterfactual Robustness rate 0.8 & 82.96 & 33.57 & 47.79  \\
%              &Diversity Robustness&  78.56 & 76.41 & 77.47 \\
%               &Negative Awareness(all noise test)& 84.12 & 83.07 & 83.59\\
%                &llama3-8b TopK-Contriever~\cite{izacard2021unsupervised}&87.13 & 86.68 & \textbf{86.91} \\
%             \hline
%              \multirow{4}*{GIT}&Labeled Database Requirement&    2.29 & 0.65 & 1.01  \\
%               &Counterfactual Robustness rate 0.2 &    74.50 & 71.61 & 73.03 \\
%               &Counterfactual Robustness rate 0.8 &   74.84 & 74.84 & 74.84\\
%              &Diversity Robustness&   74.88 & 65.38 & 69.80   \\
%               &Negative Awareness(all noise test)&   75.22 & 74.41 & 74.81\\
%                 & medllama13b MedCPT~\cite{su2023one} & 75.65 & 74.84 & \textbf{75.24}   \\ 
%            \bottomrule
% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for four testbed}
% \label{con:Model main performance}
 
% \end{table*}






% \begin{table*}[ht]
%       \Huge
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.94\textwidth}{!}{%
% 	\begin{tabular} {l|c|ccc|ccc|ccc|ccc}
% 		\toprule 
        
% 		\textbf{Dataset}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {triple}& \multicolumn{3}{c}  {head entity }& \multicolumn{3}{c}  {relation} &\multicolumn{3}{c}{tail entity} \\
% 		%\hline
% 		 &Corpus & Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 \\ 
%    \hline
%         \multirow{4}*{ADE}&Unlabeled corpus& 9.76 & 9.53 & 9.65 & 83.02 & 81.03 & 82.01 & 95.19 & 92.91 & 94.04 & 12.07 & 11.78 & 11.93 \\
         
%           &Counterfactual corpus (20\%) &  41.41 & 41.31 & 41.36 & 83.25 & 83.05 & 83.15 & 94.73 & 94.51 & 94.62 & 49.46 & 49.34 & 49.40    \\
%               &Counterfactual corpus (80\%) &  41.94 & 36.90 & 39.26 & 83.62 & 73.57 & 78.27 & 95.84 & 84.32 & 89.71 & 50.11 & 44.08 & 46.90   \\
%               &Counterfactual corpus (100\%) &  25.60 & 25.59 & 25.59 & 65.85 & 65.82 & 65.84 & 65.15 & 65.12 & 65.13 & 37.48 & 37.46 & 37.47  \\
%              &Diversity labeled corpus&  11.21 & 9.15 & 10.08 & 82.17 & 67.09 & 73.87 & 94.19 & 76.90 & 84.67 & 14.15 & 11.55 & 12.72  \\
%               % &NNegative Awareness(all noise test&  25.60 & 25.59 & 25.59 & 65.85 & 65.82 & 65.84 & 65.15 & 65.12 & 65.13 & 37.48 & 37.46 & 37.47  \\
%                &LLaMA2-13B Contriever&\textbf{36.07} & \textbf{36.06} & \textbf{36.06} & 79.76 & 79.72 & 79.74 & 93.80 & 93.76 & 93.78 & 48.99 & 48.97 & 48.98 \\
%                &No Retriever& 34.94 & 34.79 & 34.86 & 83.64 & 83.29 & 83.46 & 95.29 & 94.88 & 95.08 & 42.10 & 41.92 & 42.01 \\
%             \hline
%              \multirow{4}*{ChemProt}&Labeled Database Requirement&   75.56 & 69.14 & 72.21 & 97.77 & 89.47 & 93.44 & 90.34 & 82.66 & 86.33 & 84.11 & 76.96 & 80.38   \\
%               &Counterfactual Robustness rate 0.2 &  74.22 & 66.90 & 70.37 & 98.23 & 88.54 & 93.13 & 91.51 & 82.49 & 86.77 & 81.90 & 73.82 & 77.65   \\
%               &Counterfactual Robustness rate 0.8 & 82.96 & 33.57 & 47.79 & 98.06 & 39.67 & 56.49 & 93.03 & 37.64 & 53.59 & 89.72 & 36.30 & 51.69 \\
%              &Diversity Robustness&  78.56 & 76.41 & 77.47 & 98.15 & 95.46 & 96.79 & 89.74 & 87.29 & 88.50 & 87.77 & 85.37 & 86.55  \\
%               &Negative Awareness(all noise test)& 84.12 & 83.07 & 83.59 & 97.56 & 96.34 & 96.94 & 89.10 & 87.99 & 88.54 & 94.90 & 93.72 & 94.31    \\
%                &llama3-8b TopK-Contriever~\cite{izacard2021unsupervised}&87.13 & 86.68 & \textbf{86.91} & 97.92 & 97.41 & 97.67 & 91.26 & 90.78 & 91.02 & 95.56 & 95.06 & 95.30 \\
%             \hline
%              \multirow{4}*{GIT}&Labeled Database Requirement&    2.29 & 0.65 & 1.01 & 91.60 & 25.81 & 40.27 & 81.68 & 23.01 & 35.91 & 2.29 & 0.65 & 1.01   \\
%               &Counterfactual Robustness rate 0.2 &    74.50 & 71.61 & 73.03 & 90.60 & 87.10 & 88.82 & 83.89 & 80.65 & 82.24 & 86.58 & 83.23 & 84.87  \\
%               &Counterfactual Robustness rate 0.8 &   74.84 & 74.84 & 74.84 & 90.97 & 90.97 & 90.97 & 83.01 & 83.01 & 83.01 & 88.82 & 88.82 & 88.82  \\
%              &Diversity Robustness&   74.88 & 65.38 & 69.80 & 89.66 & 78.28 & 83.58 & 83.25 & 72.69 & 77.61 & 87.19 & 76.13 & 81.29    \\
%               &Negative Awareness(all noise test)&   75.22 & 74.41 & 74.81 & 90.00 & 89.03 & 89.51 & 80.65 & 79.78 & 80.22 & 89.35 & 88.39 & 88.86  \\
%                 & medllama13b MedCPT~\cite{su2023one} & 75.65 & 74.84 & \textbf{75.24} & 90.22 & 89.25 & 89.73 & 82.39 & 81.51 & 81.95 & 90.00 & 89.03 & 89.51  \\ 
%            \bottomrule
% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for four testbed}
% \label{con:Model main performance}
 
% \end{table*}







% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.94\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|ccc|ccc}
% 		\toprule 
  
% 		&\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{PHarmKG}& \multicolumn{3}{c}{hetionet}  \\
% 		%\hline
% 		  &Approach &data source& Precision &  Recall & F1 &  Precision &  Recall & F1  \\ 	
   
% 	      \midrule
%               \multirow{4}*{LLama2-13b}&BM25~\cite{luo2023dr}  &  train & 97.60   & 97.60      &97.60     & 82.37   & 82.37    &82.37    \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train & 98.00   &  98.00    & 98.00   &   77.00& 77.00    & 77.00   \\
%             & MedCPT~\cite{li2023petailor}&  train &  97.40  &  97.40    &  97.40&  81.60  &  81.60   &  81.60  \\
%              % &random &  train &testing  &     &   & 79.88   &  79.88   & 79.88   \\
%               &no example & --  & 97.60  &   97.60  & 97.60  &  80.80  &  80.80   &  80.80  \\
%             \hline
%                \multirow{4}*{medllama13b}&BM25~\cite{luo2023dr}  &  train & 95.00   &   95.00    &    95.00 &   90.40 & 90.40    &   90.40 \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &  97.00  &    97.00  &   97.00  &   77.20 &  77.20   &   77.20 \\
%             & MedCPT~\cite{li2023petailor}&  train &   97.40    &   97.40     &  97.40      &   84.40 &   84.40  &   84.40 \\
%              % &random &  train &  running &     &   &    &     &    \\
%                &no example &  -- & 97.20  &  97.20    &97.20   &  78.54  &  78.54   &  78.54  \\
%              \hline
%         \multirow{4}*{llama3 8b}&BM25~\cite{luo2023dr}  &  train & 96.80  & 96.80    &  96.80 &  81.80  &   81.80  &   81.80 \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train & 96.60   &   96.60    &  96.60  &  73.40  &  73.40   &   73.40 \\
%             & MedCPT~\cite{li2023petailor}&  train &  97.00  &  97.00   & 97.00   & 83.00   &   83.00  &  83.00  \\
%              % &random &  train & testing   &     &   & 80.29   &  80.29    & 80.29    \\
%                &no example & --- &  97.20 & 97.20    &  97.20 &   81.80 &  81.80   &   81.80 \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction on AZ and hetionet.}
% \label{con:Model main performance}
 
% \end{table*}







% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.7\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|c|c|c}
% 		\toprule 
  
% 		% &\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{BioNLI}  \\
% 		%\hline
% 		  &Approach &data source&   Precision  & Recall&F1 \\ 	
% 	      \midrule
%               \multirow{4}*{PHarmKG}&Labeled Database Requirement&  --& 97.20    &97.20 &   97.20  \\
%             &Counterfactual Robustness rate 0.2 &  --&  97.40   &  97.40 &     97.40  \\
%               &Counterfactual Robustness rate 0.8 &  --& 97.80  & 97.80 & 97.80       \\
%              &Diversity Robustness&  --&  97.20       &  97.20  &    97.20   \\
%               &Negative Awareness(all noise test)&  --&   97.60  & 97.60 &   97.60     \\
%                &LLama2-13b TopK-Contriever&  --&  98.00 & 98.00 & 98.00      \\
%        \hline
%                \multirow{4}*{hetionet}&Labeled Database Requirement&  --&  & &     \\
%             &Counterfactual Robustness rate 0.2 &  --&       & &     \\
%               &Counterfactual Robustness rate 0.8 &  --&     & &       \\
%              &Diversity Robustness&  --&         & &    \\
%               &Negative Awareness(all noise test)&  --&     & &       \\
%                &medllama 13b   BM25&  --& 90.40  &90.40& 90.40    \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction on BioNLI}
% \label{con:Model main performance}
 
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.5\textwidth}{!}{%
% 	\begin{tabular} {l|c|c}
% 		\toprule 
  
% 		  Dataset & true negative awareness rate &fake negative awareness \\ 	
%              PHarmKG&  0.00 & 63.11  \\
% 	       hetionet&   & \\
        
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for negative awareness rate}
% \label{con:Model main performance}
 
% \end{table*}






% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.94\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|ccc|ccc}
% 		\toprule 
  
% 		&\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{AZ}& \multicolumn{3}{c}{hetionet}  \\
% 		%\hline
% 		  &Approach &data source& Precision &  Recall & F1 &  Precision &  Recall & F1  \\ 	
   
% 	      \midrule
%               \multirow{4}*{LLama2-13b}&BM25~\cite{luo2023dr}  &  train &  \textbf{63.05} &  63.05  & 63.05  & 82.37   & 82.37    &82.37    \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &   60.27 &   60.27  &  60.27 &   76.80& 76.80    & 76.80   \\
%             & MedCPT~\cite{li2023petailor}&  train &  59.58  &  59.58    &  59.58  &  81.60  &  81.60   &  81.60  \\
%              &random &  train &  61.94 &  61.94   &  61.94 & 79.88   &  79.88   & 79.88   \\
%             \hline
%                \multirow{4}*{medllama13b}&BM25~\cite{luo2023dr}  &  train &  52.36 & 52.36    &52.36   &    &     &    \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &   59.58 &   59.58  &   59.58&    &     &    \\
%             & MedCPT~\cite{li2023petailor}&  train &  60.13   &  60.13    &    60.13 &    &     &    \\
%              &random &  train & 45.56  &  45.56   & 45.56  &    &     &    \\
%              \hline
%         \multirow{4}*{llama3 8b}&BM25~\cite{luo2023dr}  &  train & wait for test  &     &   &    &     &    \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &  wait for test &     &   &    &     &    \\
%             & MedCPT~\cite{li2023petailor}&  train &  wait for test &     &   &    &     &    \\
%              &random &  train &  running &     &   &    &     &    \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction on AZ and hetionet.}
% \label{con:Model main performance}
%  
% \end{table*}


% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.94\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|ccc|ccc}
% 		\toprule 
  
% 		&\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{ade-corpus-2}& \multicolumn{3}{c}{semed-triple-classification}  \\
% 		%\hline
% 		  &Approach &data source& Precision &  Recall & F1 &  Precision &  Recall & F1  \\ 	
   
% 	      \midrule
%               \multirow{4}*{LLama2-13b}&BM25~\cite{luo2023dr}  &  train & 95.40  &95.40      & 95.40   &  75.50  &   75.50   &  75.50 \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train & 96.60   & 96.60     &  96.60  & 79.33  &    79.33 &     79.33 \\
%             & MedCPT~\cite{li2023petailor}&  train & 96.80    &  96.80   & 96.80   & 78.50    &  78.50    &     78.50 \\
%              % &random &  train &  96.20  & 96.20      & 96.20    &   running &     &    \\
%                &no example &   & 96.40  & 96.40    &  96.40 &   77.66  & 77.66   & 77.66  \\
%             \hline
%                \multirow{4}*{medllama13b}&BM25~\cite{luo2023dr}  &  train & 95.60   & 95.60    &  95.60 &  72.67  &   72.67  &   72.67  \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &  95.60  &  95.60   &  95.60 &  77.66 & 77.66   & 77.66   \\
%             & MedCPT~\cite{li2023petailor}&  train & 95.40 & 95.40    & 95.40  &76.16    &  76.16    &   76.16  \\
%              % &random &  train &94.00   & 94.00     & 94.00   &  running  &     &    \\
%                &no example &    & 95.40  &  95.40   & 95.40  &   64.00 &    64.00 &  64.00  \\
%              \hline
%         \multirow{4}*{llama3 8b}&BM25~\cite{luo2023dr}  &  train &94.80   & 94.80    & 94.80   & 75.50  &   75.50    &  75.50    \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train & 94.60  &  94.60    & 94.60   &   75.83 &  75.83 &75.83      \\
%             & MedCPT~\cite{li2023petailor}&  train & 95.40 & 95.40    & 95.40  & 74.67 &  74.67   & 74.67   \\
%              % &random &  train &  testing &     &   &   running &     &    \\
%                &no example &   -- &93.80   & 93.80      & 93.80    &   73.16 &   73.16   &  73.16   \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction on ade-corpus-2 and semed-triple-classification}
% \label{con:Model main performance}
 
% \end{table*}





% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.7\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|c|c|c}
% 		\toprule 
  
% 		% &\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{BioNLI}  \\
% 		%\hline
% 		  &Approach &data source&   Precision  & Recall&F1 \\ 	
% 	      \midrule
%               \multirow{4}*{ade-corpus-2}&Labeled Database Requirement&  --&  94.80   &94.80  &   94.80   \\
%             &Counterfactual Robustness rate 0.2 &  --&   95.80   &95.80  &   95.80   \\
%               &Counterfactual Robustness rate 0.8 &  --&    95.00   & 95.00  &   95.00      \\
%              &Diversity Robustness&  --&   96.20     &96.20   & 96.20     \\
%               &Negative Awareness (all noise test)&  --&   96.80   & 96.80   &    96.80  \\
%                &LLama2-13b MedCPT&  --&  96.80 & 96.80& 96.80    \\
%                 &LLama2-13b&  --&  96.40   & 96.40& 96.40   \\
%        \hline
%                \multirow{4}*{semed-triple-classification}&Labeled Database Requirement&  --&6.83   & 6.83 &  6.83    \\
%             &Counterfactual Robustness rate 0.2 &  --&   73.33     &  73.33 &  73.33     \\
%               &Counterfactual Robustness rate 0.8 &  --&    75.66  & 75.66 &  75.66      \\
%              &Diversity Robustness&  --&   75.33      & 75.33  &  75.33    \\
%               &Negative Awareness(all noise test)&  --& 77.66     & 77.66&    77.66   \\
%                &llama2-13b   contriver &  --& 79.33  &79.33  & 79.33    \\
%                  &llama2-13b    &  --& 77.66  &77.66   & 77.66   \\
%            \bottomrule

% 	\end{tabular}
% }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction}
% \label{con:Model main performance}
 
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|c|c}
% 		\toprule 
  
% 		  Dataset & true negative awareness rate  & fake negative awareness rate \\ 	
%              ade-corpus-2& 68.75    &  70.45  \\
% 	    semed-triple-classification&1.49   &  99.35  \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{awareness rate}
% \label{con:Model main performance}
 
% \end{table*}
  


% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.94\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|ccc|ccc}
% 		\toprule 
  
% 		&\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{PubmedQA(or others)}& \multicolumn{3}{c}{MedMCQA}  \\
% 		%\hline
% 		  &Approach &data source& Precision &  Recall & F1 &  Precision &  Recall & F1  \\ 	
   
% 	      \midrule
%               \multirow{4}*{LLama2-13b}&BM25~\cite{luo2023dr}  &  train &   &     &   &  40.38  &  40.49   & 40.42   \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &   &     &   &  35.53  &  35.52   &  35.52  \\
%             & MedCPT~\cite{li2023petailor}&  train &   &     &   &  36.78  &  36.93   &  36.80  \\
%              &no example &  train &   &     &   &    &     &    \\
%             \hline
%                \multirow{4}*{medllama13b}&BM25~\cite{luo2023dr}  &  train &   &     &   &  37.81  & 37.96    &  37.86  \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &   &     &   &  29.82  &   29.75  &  29.77  \\
%             & MedCPT~\cite{li2023petailor}&  train &   &     &   &  33.86  &  34.04   &  33.88  \\
%              &no example &  train &   &     &   &    &     &    \\
%              \hline
%         \multirow{4}*{llama3 8b}&BM25~\cite{luo2023dr}  &  train &   &     &   &  37.73  &  38.90   & 37.79   \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &   &     &   &  28.11  &  28.12   &  28.11  \\
%             & MedCPT~\cite{li2023petailor}&  train &   &     &   &  31.57  &  31.82   &  31.56  \\
%              % &random &  train &   &     &   &    &     &    \\
%                &no example &  train &   &     &   &    &     &    \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for Medical question answering on PubmedQA and MedMCQA, (train set length=34994)}
% \label{con:Model main performance}
 
% \end{table*}



% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.7\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|c|c|c}
% 		\toprule 
  
% 		% &\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{BioNLI}  \\
% 		%\hline
% 		  &Approach &data source&   Precision  & Recall&F1 \\ 	
% 	      \midrule
%               \multirow{4}*{MedMCQA}&Labeled Database Requirement&  --&  & &     \\
%             &Counterfactual Robustness rate 0.2 &  --&       & &     \\
%               &Counterfactual Robustness rate 0.8 &  --&     & &       \\
%              &Diversity Robustness&  --&         & &    \\
%               &Negative Awareness&  --&     & &       \\
%                &&  LLama2-13b  BM25& 40.38  &  40.49  &  40.42   \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction}
% \label{con:Model main performance}
 
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|c|c}
% 		\toprule 
  
% 		  Dataset & true negative awareness rate  & fake negative awareness rate \\ 	
%              MedMCQA&     &    \\
% 	       % semed-triple-classification&    \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{awareness rate}
% \label{con:Model main performance}
 
% \end{table*}
  


% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.7\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|c}
% 		\toprule 
  
% 		&\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{BioNLI}  \\
% 		%\hline
% 		  &Approach &data source&  Macro-avg F1  \\ 	
% 	      \midrule
%               \multirow{4}*{LLama2-13b}&BM25~\cite{luo2023dr}  &  train     & 45.10  \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train   &  35.12    \\
%             & MedCPT~\cite{li2023petailor}&  train     &  69.21   \\
%              % &random &  train &   67.26    \\
%              &no-example &   &      62.62 \\
%             \hline
%                \multirow{4}*{medllama13b}&BM25~\cite{luo2023dr}  &  train &    48.81   \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train &      53.07  \\
%             & MedCPT~\cite{li2023petailor}&  train &    53.68     \\
%              % &random &  train &     60.34   \\
%               &no-example &   &    61.07\\
%              \hline
%         \multirow{4}*{llama3 8b}&BM25~\cite{luo2023dr}  &  train & 19.17     \\
%             &TopK-Contriever~\cite{izacard2021unsupervised}&  train & 63.85   \\
%             & MedCPT~\cite{li2023petailor}&  train &  56.89     \\
%              % &random &  train &        \\
%               &no-example &   & 6.71      \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction on BioNLI}
% \label{con:Model main performance}
 
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.7\textwidth}{!}{%
% 	\begin{tabular} {l|l|c|c}
% 		\toprule 
  
% 		% &\multicolumn{1}{c}  {}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{BioNLI}  \\
% 		%\hline
% 		  &Approach &data source&   F1 \\ 	
% 	      \midrule
%               \multirow{4}*{BioNLI}&Labeled Database Requirement&  -- &  10.91   \\
%             &Counterfactual Robustness rate 0.2 &  --&     47.76     \\
%               &Counterfactual Robustness rate 0.8 &  --&  64.63       \\
%              &Diversity Robustness&  --&    80.32      \\
%               &Negative Awareness&  --& 46.46         \\
%                &LLama2-13b MedCPT &  --&    69.21       \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for link prediction}
% \label{con:Model main performance}
 
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|c|c}
% 		\toprule 
  
% 		  Dataset & true negative awareness rate  & fake negative awareness  rate\\ 	
%              BioNLI&   0 &0.38   \\
% 	       % semed-triple-classification&    \\
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{awareness rate}
% \label{con:Model main performance}
 
% \end{table*}

% true-noise:0, all_noise: 1633, $0 /1633 = 0$  fake noise, 18, all noise right 4675,$18 /4675=0$}

% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.94\textwidth}{!}{%
% 	\begin{tabular} {l|c|ccc|ccc}
% 		\toprule 
  
% 		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {NCBI}& \multicolumn{3}{c}  {BC5CDR}  \\
% 		%\hline
% 		 Approach &data source& Precision &  Recall & F1 &  Precision &  Recall & F1  \\ 
% 		%\hline	
   
% 	      \midrule
%               % \textbf{from train} &  &     &    &  &   &   &      &   &    &   &   &    &   \\
%                random &  train &   &     &   &    &     &    \\
%             BM25~\cite{luo2023dr} &  train &   &     &   &    &     &    \\
%             % TopK+MDL~\cite{wu2023self}  &      &    &  &   &   &      &   &    &   &   &    &   \\
%             TopK-Contriever~\cite{izacard2021unsupervised}&  train &   &     &   &    &     &    \\
%             % RA-KNN-n~\cite{li2023petailor}&      &    &  &   &   &      &   &    &   &   &    &   \\
%             % Instructor~\cite{su2023one} &  train &   &     &   &    &     &    \\
%              MedCPT~\cite{li2023petailor} &  train &   &     &   &    &     &    \\
           
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for NER on NCBI and BC5CDR.}
% \label{con:Model main performance}
%  
% \end{table*}




\subsection{Baselines}












\subsection{Results and Discussion}
\label{con:discussuion_triple}




\subsection{Analysis}


% \begin{figure}[t]
%         \centering
%         \includegraphics[width=0.98\columnwidth]{chuck_number.pdf}
% 	\caption{  \textsc{PeTailor} performance with different  chunk length ($m$) in the triple extraction task. P is Precision, R is Recall and F is F1-score.
%  }
% 	\label{con:chunk_number_triple}
% \end{figure}


\subsubsection{Ablation Experiments}



==> result_zero_shot_6_2.tex <==


\section{Experiments}
\label{experiments}


\subsection{Settings}
2,676,642 notes, 7.27G. 

515,524 report, 536.85M.




\subsection{Baselines}



\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc|c}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}&  F1\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 & Average\\
	      \midrule
        % Mamba 2.7 B~\cite{gu2023mamba} &     &     &    &     &    &     &       \\
        PMC LLaMA 7B~\cite{wu2023pmc} &   88.61/0.00    &     88.61/0.00    &  88.61/0.00      & 90.36 /0.00     &  90.36/0.00   &     90.36/0.00   & 93.26/0.00   &  93.26/0.00  &  93.26/0.00   &  90.74/0.00\\
         Medalpaca 7B~\cite{han2023medalpaca} &   89.28 /0.00    &  89.28/0.00      &  89.28/0.00     &   91.27/0.00    &  91.27/0.00    &  91.27/0.00       &93.89/0.00   & 93.89/0.00   & 93.89/0.00    &91.48/0.00  \\
          LLAMA-2 7B~\cite{han2023medalpaca} &  89.18/0.00     &   89.18/0.00        &  89.18/0.00        &  90.83/3.09     &   90.83/3.09    &   90.83/3.09       &  93.53/10.80  &93.53/10.80     & 93.53/10.80    & 91.18 \\
   Mistral 1*7B~\cite{jiang2023mistral} &    89.47/0.00     &     89.47/0.00      &   89.47/0.00       &   91.30/3.28   & 91.30/3.28     & 91.30/3.28        & 94.19/10.88   &  94.19/10.88 &   94.19/10.88 & 91.65\\
     Mistral 8*7B~\cite{jiang2023mistral} &   90.23/0.00      &     90.23/0.00    &     90.23 /0.00  &    92.05/3.92    &92.05/3.92      &   92.05/3.92      & 94.50/13.47    & 94.50/13.47    &94.50 /13.47     &  \textbf{92.26} \\
      Bio-Mistral 7B~\cite{labrak2024biomistral}&   88.90/0.85     &    88.90/0.85    &     88.90/0.85  & 91.05/4.70      &91.05/4.70      &  91.05/4.70       &   93.79/14.80  &93.79/14.80   &  93.79/14.80 &  91.24 \\
 LLama3 8B~\cite{} &    89.94/0.00    &    89.94/0.00    &  89.94/0.00     &  91.75/1.30     &   91.75/1.30      &   91.75/1.30         & 94.34/5.67   & 94.34/5.67  &   94.34/5.67& \textbf{92.01} \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc} &    88.80/13.57    &    88.80/13.57    &  88.80 /13.57    &   90.87/11.02    &  90.87/11.02    &  90.87/11.02      & 93.31 /21.55   &  93.31/21.55 &  93.31 /21.55  &  90.99\\
                PMC LLaMA 13B~\cite{wu2023pmc}&   87.95/0.00    &  87.95/0.00           &   87.95/0.00         &  89.64/1.14     &   89.64/1.14    &  89.64 /1.14       &  92.58/4.55  &  92.58/4.55 &92.58/4.55   &  90.06\\
                Medalpaca 13B~\cite{han2023medalpaca} &  88.61/0.00      &   88.61/0.00        &    88.61/0.00     & 90.37 /0.17     &    90.37/0.17 &  90.37/0.17        &92.94/0.72    &  92.94/0.72 &  92.94/0.72 & 90.64 \\
                 LLaMA2 13B~\cite{touvron2023llama}&    89.85/4.46    &   89.85 /4.46     &    89.85/4.46    &  91.54/6.07     &  91.54/6.07      & 91.54/6.07          &  94.21/15.30   &   94.21/15.30   &   94.21/15.30   & \textbf{ 91.86} \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} &    90.04/0.00    &    90.04/0.00    &   90.04/0.00    & 91.62/3.50     &91.62/3.50     &   91.62/3.50      &93.98/11.30     &93.98/11.30    & 93.98/11.30    &   91.88\\
                % MEDITRON-70B~\cite{chen2023mtestingeditron} &      &        &      &     &   &     & \\
                    Llama3-OpenBioLLM-70B&  88.33/1.52      &   88.33/1.52     &  88.33/1.52     &   90.02/4.73    &           90.02/4.73  & 90.02 /4.73  &   93.15/14.74  &  93.15/14.74  &   93.15/14.74    & 90.50 \\
                ClinicalCamel-70B~\cite{toma2023clinical} &  92.02/1.71      &  92.02/1.71       &    92.02/1.71    &   93.62/5.58    &   93.62/5.58   &    93.62/5.58     &  95.52/17.25  &  95.52/17.25   &   95.52/17.25  &  \textbf{93.72}  \\
                \hline
                 Ours-test1 (pre-train: mixtural, fine-tuning: mixtrual) &    89.37/0.09    &  89.37/0.09       &  89.37/0.09     &   91.98/3.43    &91.98/3.43     &  91.98/3.43      &  93.98/11.18 & 93.98/11.18   &   93.98/11.18 & 91.78  \\
                  Ours-test2 (pre-training biomixtural, fine-tuning: mixtrual ) & 84.06       &  84.06      &  84.06     & 86.35       &  86.35      &    86.35      &   88.76 &    88.76 &   88.76  &86.39     \\
                 Ours-test3 (pre-training biomixtural, fine-tuning: biomixtrual ) & 88.90      & 88.90      & 88.90     & 91.20       &    91.20   &      91.20   &  93.81   & 93.81     & 93.81     & 91.30    \\    
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of  breast Cancer Diagnosis  (full/zero shot)}
\label{con:Model_performance_Cancer_plan}
\vspace{-1mm}
\end{table*}




\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc|c}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}&\multicolumn{1}{c}  {F1}\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 &  Average \\
	      \midrule
        PMC LLaMA 7B~\cite{wu2023pmc} &  47.04/0.00    &   47.04/0.00    &    47.04/0.00  &   56.41/0.00    & 56.41/0.00   &56.41/0.00      & 66.98/0.00 & 66.98/0.00  & 66.98/0.00 &  56.81\\
         Medalpaca 7B~\cite{han2023medalpaca} &   41.75/0.09   &  41.75/0.09    &   41.75/0.09  &   50.16/0.93  & 50.16/0.93   & 50.16/0.93     &62.07/3.47  &62.07/3.47&62.07/3.47  &51.33\\
          LLAMA-2 7B~\cite{han2023medalpaca} &  33.18/0.00    &     33.18/0.00   &   33.18/0.00   & 42.80/0.64    &  42.80/0.64  &   42.80 /0.64  & 55.09/2.76 & 55.09/2.76& 55.09/2.76   &43.96 \\
   Mistral 1*7B~\cite{jiang2023mistral} & 45.40/0.00    & 45.40/0.00 &   45.40/0.00 &  54.29/1.11    & 54.29/1.11   &   54.29/1.11    &  65.52/4.52  &  65.52/4.52&  65.52/4.52  &  55.07\\
     Mistral 8*7B~\cite{jiang2023mistral} & 51.32/0.00     &51.32/0.00         &   51.32/0.00    & 59.35/0.84    & 59.35/0.84   & 59.35 /0.84    & 69.70/4.36  & 69.70/4.36     & 69.70/4.36  &  60.12\\
      Bio-Mistral 7B~\cite{} & 62.26/0.00   & \textbf{ 62.26}/0.00   &  62.26/0.00  &  68.40/1.73    &  68.40/1.73   &  68.40/1.73      &76.02/4.85  &76.02/4.85   & 76.02/4.85 &68.89 \\
 LLama3 8B~\cite{} &  51.60/0.00  &  51.60/0.00   &    51.60/0.00  &  60.13/0.00    &  60.13/0.00  &  60.13/0.00    &  69.97/0.22   & 69.97/0.22    &  69.97/0.22  & 60.57  \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc} &   39.02/0.00   &39.02/0.00     & 39.02/0.00     &48.98/0.00       &  48.98/0.00 &  48.98/0.00    &60.63/0.03  &60.63/0.03&60.63/0.03  &49.54 \\
                PMC LLaMA 13B~\cite{wu2023pmc} &    54.97/0.00   & 54.97/0.00     &  54.97/0.00       &62.56/1.05     &  62.56/1.05   & 62.56/1.05       & 71.06/4.52  &  71.06/4.52  &  71.06/4.52  &62.86 \\
                Medalpaca 13B~\cite{han2023medalpaca} &    40.66/0.00    & 40.66 /0.00   &   40.66/0.00    & 50.58/0.00      & 50.58/0.00   &   50.58/0.00        &62.40/0.01  & 62.40/0.01  &  62.40/0.01  & 51.21 \\
                 LLaMA2 13B~\cite{touvron2023llama} & 45.76/0.46      &   45.76/0.46     &  45.76/0.46    &  54.70/1.30     &54.70/1.30   &  54.70/1.30    &   65.80/3.48  &65.80/3.48    & 65.80/3.48 & 55.42 \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} &50.23/0.00     &  50.23/0.00        &  50.23/0.00    & 59.63/1.03     & 59.63/1.03  &   59.63/1.03   & 69.25/3.93   &  69.25/3.93  &  69.25/3.93 & 59.70\\
                % MEDITRON-70B~\cite{chen2023meditron} &      &        &      &     &   &     & \\
                   ClinicalCamel-70B& 54.60/0.09   &   54.60/0.09       &   54.60/0.09    &  63.34/2.80    & 63.34/2.80  &   63.34/2.80   & 72.73/8.77   & 72.73/8.77 &72.73/8.77 & 63.55\\
               
                
                Llama3-OpenBioLLM-70B&   54.42/0.27    &   54.42/0.27        & 54.42/0.27      &   62.36/2.52    & 62.36/2.52&   62.36/2.52  & 71.65/7.65   &  71.65/7.65 &  71.65/7.65 &62.81\\
                \hline
                 Ours  -test1 (pre-train: mixtural, fine-tuning: mixtrual)  &  79.85    &  79.85      & 79.85   &  83.66    &83.66  &     83.66 &  88.51  & 88.51    &  88.51   &  84.00 \\
                   Ours  -test1 (pre-train: mixtural, fine-tuning: bio-mixtrual) &   \textbf{83.50}/0.00    &   \textbf{83.50 }/0.00      &   \textbf{83.50}/0.00    & 86.60 /0.70     &86.60/0.70  &  86.60 /0.70   &   90.34/2.94   &90.34/2.94  &90.34/2.94  &   \textbf{86.81}\\
                     Ours-test2 (pre-training biomixtural, fine-tuning: mixtrual ) &  79.58     &    79.58   &   79.58   &   83.67    &   83.67     &   83.67       &  88.40   &  88.40    &  88.40    &  83.88   \\
                 Ours-test3 (pre-training biomixtural, fine-tuning: biomixtrual ) &  79.49       &    79.49   & 79.49     &     83.74   &  83.74    &     83.74   & 88.67  & 88.67    &88.67     &  83.97   \\
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of  lung  and breast Cancer Diagnosis}
\label{con:Model_performance_Cancer_plan}
\vspace{-1mm}
\end{table*}






\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{1\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc|c}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Exact Match} &\multicolumn{3}{c}  {BLEU-2}&\multicolumn{3}{c}  {ROUGE-L}&\multicolumn{1}{c}  {F1}\\
		%\hline
		 Approach & Precision &  Recall & F1 & Precision &  Recall & F1 & Precision &  Recall & F1 &  Average \\
	      \midrule
        PMC LLaMA 7B~\cite{wu2023pmc} &   10.61    & 10.61      &  10.61   & 64.52      &64.52    &  64.52   & 74.08   & 74.08  & 74.08  \\
         Medalpaca 7B~\cite{han2023medalpaca} & 11.11    &    1.11     &    11.11  & 65.26     & 65.26   & 65.26      & 74.69  &  74.69  &  74.69  &   \\
          LLAMA-2 7B~\cite{han2023medalpaca} &  8.51  &   8.51     &  8.51   &    62.28   &  62.28 &  62.28    & 72.09  &  72.09  & 72.09   &   \\
   Mistral 1*7B~\cite{jiang2023mistral} &   14.01    &  14.01       &  14.01    & 67.30      &    67.30   & 67.30  &  75.94  & 75.94  &75.94   \\
     Mistral 8*7B~\cite{jiang2023mistral}& testing      &        &     &      &   &      &  &   &   &   \\
      Bio-Mistral 7B~\cite{} &     13.71   &     13.71    &   13.71   &  67.85     &   67.85  &    67.85    & 76.61  &  76.61 &  76.61 &   \\
 LLama3 8B~\cite{} &  12.31   & 12.31        &  12.31    &  65.60     &  65.60  & 65.60      & 74.26  &   74.26 & 74.26   &   \\
                \hline
                MedLLaMA 13B~\cite{wu2023pmc}&  11.91      &    11.91     & 11.91     &   66.48    &    66.48 &   66.48     & 75.59  & 75.59  & 75.59  &   \\
                PMC LLaMA 13B~\cite{wu2023pmc}&  12.11   &  12.11      &   12.11  &66.34       & 66.34    &  66.34      & 75.62  &  75.62  &   75.62 &   \\
                Medalpaca 13B~\cite{han2023medalpaca} &  12.11    &     12.11     &   12.11    &  65.66     &  65.66 &   65.66   & 74.55  & 74.55   &  74.55  &   \\
                 LLaMA2 13B~\cite{touvron2023llama} &  9.51       &  9.51       &  9.51    & 64.36      &  64.36 & 64.36    & 73.93  & 73.93   & 73.93   &   \\
                 \hline
                  LLaMA2 70B~\cite{touvron2023llama} &   testing 3     &        &     &      &   &      &  &   &   &   \\
                % MEDITRON-70B~\cite{chen2023meditron} &      &        &      &     &   &     & \\
                   ClinicalCamel-70B&  testing   4   &        &     &      &   &      &  &   &   &   \\
               
                
                Llama3-OpenBioLLM-70B&  testing 5     &        &     &      &   &      &  &   &   &   \\
                \hline
                 Ours  -test1 (pre-train: mixtural, fine-tuning: mixtrual) &    15.32     &      15.32  & 15.32    &  70.71    &  70.71  & 70.71      & 79.00  &  79.00  &79.00    &   \\
                   Ours  -test1 (pre-train: mixtural, fine-tuning: bio-mixtrual) &   15.72      & 15.72        & 15.72     &  71.09     &  71.09  &  71.09     &79.41  & 79.41  &  79.41 &   \\
                     Ours-test2 (pre-training biomixtural, fine-tuning: mixtrual ) &        &      &     &       &      &        &    &     &     &     \\
                 Ours-test3 (pre-training biomixtural, fine-tuning: biomixtrual ) &        &      &     &       &      &        &    &     &     &     \\
           % Med-Alpaca &     &     &   \\
           \bottomrule
	\end{tabular}
  }
\vspace{+2mm}
\caption{Results of  lung  and breast Cancer Diagnosis, new token 1000, max token 4000, generation slow}
\label{con:Model_performance_Cancer_plan}
\vspace{-1mm}
\end{table*}





% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|ccc|ccc|ccc}
% 		\toprule 
  
% 		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Breast cancer}& \multicolumn{3}{c}  {lung cancer} & \multicolumn{3}{c}  {other cancer} \\
% 		%\hline
% 		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 \\
   
% 	      \midrule
%                 MedLLaMA 13B~\cite{wu2023pmc} &     &    &     &   &  &  &  &  &  \\
%                  LLaMA2 13B~\cite{touvron2023llama} &     &     &       &     & &    & &   & \\
%                 Mistral-7B~\cite{jiang2023mistral} &     &     &       &     & &    & &   & \\
%                  Mamba 2.7 B~\cite{gu2023mamba} &     &     &       &     & &    & &   & \\
%            Med-Alpaca &     &     &       &     & &    & &   & \\
           
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for cancer QA, few-shot result}
% \label{con:Model_performance_Chem_DDI_GIT}
% \vspace{-1mm}
% \end{table*}




% \begin{table*}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.8\textwidth}{!}{%
% 	\begin{tabular} {l|ccc|ccc|ccc}
% 		\toprule 
  
% 		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Breast cancer}& \multicolumn{3}{c}  {lung cancer} & \multicolumn{3}{c}  {other cancer} \\
% 		%\hline
% 		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 \\
   
% 	      \midrule
%                 MedLLaMA 13B~\cite{wu2023pmc} &     &    &     &   &  &  &  &  &  \\
%                  LLaMA2 13B~\cite{touvron2023llama} &     &     &       &     & &    & &   & \\
%                 Mistral-7B~\cite{jiang2023mistral} &     &     &       &     & &    & &   & \\
%                  Mamba 2.7 B~\cite{gu2023mamba} &     &     &       &     & &    & &   & \\
%            Med-Alpaca &     &     &       &     & &    & &   & \\
           
%            \bottomrule

% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of various approaches for cancer QA, zero-shot result}
% \label{con:Model_performance_Chem_DDI_GIT}
% \vspace{-1mm}
% \end{table*}







\subsection{Results and Discussion}
\label{con:discussuion_triple}




\subsection{Analysis}




\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=2in]{cancer_LLM_patient_1.pdf}
    }
     \subfigure[]{
        \includegraphics[width=2.5in]{cancer_LLM_patient_2.pdf}
    }
    
    % \quad    %用 \quad 来换行
    \caption{Patients Statistics}
   \label{con:ablated models}
\end{figure}


\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=2in]{cancer_LLM_patient_notes_1.pdf}
    }
     \subfigure[]{
        \includegraphics[width=3in]{cancer_LLM_patient_notes_2.pdf}
    }
    
    % \quad    %用 \quad 来换行
    \caption{clinical notes }
   \label{con:ablated models}
\end{figure}



\subsubsection{Ablation Experiments}


